MathBench: Evaluating the Theory and Application Proficiency of LLMs with a Hierarchical Mathematics Benchmark

Recent advancements in large language models (LLMs) have showcased significant improvements in mathematics. However, traditional math benchmarks like GSM8k offer a unidimensional perspective, falling short in providing a holistic assessment of the LLMs' math capabilities. To address this gap, we introduce MathBench, a new benchmark that rigorously assesses the mathematical capabilities of large language models. MathBench spans a wide range of mathematical disciplines, offering a detailed evaluation of both theoretical understanding and practical problem-solving skills. The benchmark progresses through five distinct stages, from basic arithmetic to college mathematics, and is structured to evaluate models at various depths of knowledge. Each stage includes theoretical questions and application problems, allowing us to measure a model's mathematical proficiency and its ability to apply concepts in practical scenarios. MathBench aims to enhance the evaluation of LLMs' mathematical abilities, providing a nuanced view of their knowledge understanding levels and problem solving skills in a bilingual context. The project is released at https://github.com/open-compass/MathBench .

==> backup/experiment.tex <==
\section{Experiments and Analysis}

\subsection{Configuration}

\paragraph{Evaluation Protocols. }
We employ CircularEval (CE)~\citep{mmbench} and Perplexity (PPL) as our principal evaluation methodology for Chat and Base models respectively.
CE systematically assesses an $N$-option multi-choice question by evaluating it $N$ times, each time permuting the order of the options. 

% removed
% To ensure uniformity across evaluations, we set the maximum output length at 512 tokens and use the greedy decoding strategy for all LLMs. 
% We adopt the few-shot setting for open-ended questions and the zero-shot setting for multi-choice questions on Chat models, few-shot for Base models in PPL evaluation.

To maintain consistency in evaluations, we standardized the maximum output length to 2048 tokens and employed a greedy decoding strategy for all Large Language Models (LLMs). For open-ended questions, we utilized a few-shot CoT setting, whereas for multiple-choice questions on Chat models, we implemented a zero-shot CoT approach. In the case of Base models during PPL evaluation, a few-shot setting was adopted.

\paragraph{Evaluated Models. }
Our evaluation encompasses both closed-source commercial LLMs and open-source LLMs, covering more than $20$ models. 
Based on MathBench, we deliver a thorough evaluation of the capabilities of current LLMs.
We list all evaluated LLMs below:

% \begin{enumerate}[leftmargin=*,topsep=0.5ex,itemsep=-0.5ex,partopsep=0.75ex,parsep=0.75ex,partopsep=0pt,wide]

\noindent$\bullet$ Closed-source models: GPT-3.5 and GPT-4\footnote{GPT-4 version: \texttt{gpt-4-0125-preview and GPT-4o-2024-05-13}; GPT-3.5 version: \texttt{gpt-3.5-turbo-0125}}from Openai, Qwen-Max\footnote{\url{https://help.aliyun.com/zh/dashscope/create-a-chat-foundation-model?spm=a2c4g.11186623.0.0.581c64d16b7Azw}}, DeepSeek-V2, GLM4\footnote{\url{https://open.bigmodel.cn/dev/howuse/glm4}} and Anthropic Claude-3-Opus\footnote{\url{https://www.anthropic.com/news/claude-3-family}}.
% Qwen-max google-api

\noindent$\bullet$ OpenSource LLMs: We evaluate a wide spectrum of LLMs, including Llama3\cite{touvron2023llama2}, Qwen \cite{bai2023qwen}, InternLM2 \cite{team2023internlm}, Yi \footnote{\url{https://github.com/01-ai/Yi}}, Baichuan2~\citep{yang2023baichuan},  DeepSeek\cite{deepseek}, Mixtral\cite{jiang2024mixtral}and ChatGLM3 \cite{zeng2022glm}.

\noindent$\bullet$ OpenSource Math LLMs: Llemma\cite{azerbayev2023llemma}, MetaMath-llemma\cite{MetaMath}, DeepSeek-Math\cite{deepseekmath}, MAmmoTH\cite{mammoth} and InternLM2-Math\citep{ying2024internlmmath}.
% \end{enumerate}

\subsection{Main Results}
We showcase the principal outcomes of MathBench in \Cref{tab: apllication_theory_chat_result}, detailing the application-oriented aspects in (\textit{MathBench-A}), and the theoretical components in (\textit{MathBench-T}).

% \input{tabs/application_tab}
% \input{tabs/theory_tab}

\input{tabs/application_theory_tab_2k}


\subsubsection{MathBench-A}

Among all evaluated models on the application part of MathBench, GPT-4 achieves the highest overall average score, specifically excelling in the more challenging \textit{Middle}, \textit{High}, and \textit{College} stages. Following GPT-4, Claude-3-Opus outperforms in basic arithmetic operations, including \textit{Arithmetic} and \textit{Primary} stages.
The best LLM for open-source is Qwen-72B-Chat, its outstanding performance distinguishes itself as the leading player among all open-source models. 
We also notice that DeepSeek-Math-7B-RL, an LLM dedicated to mathematical tasks, secures its position as the best open-source model in mathematics,   
which is impressive given its small parameter size.

Among open-source chat models, 
performances across models with $\sim$7B, $\sim$20B, and $\sim$70B parameter size reveal distinct capabilities:

\noindent \textbf{$\sim$7B Chat Models. }
InternLM2-Chat-7B emerges as the superior model at the $\sim$7B scale and outperforms other 7B Chat models across all stages.
It's noteworthy that, as the difficulty of problems increases, the gap between InternLM2-Chat-7B and other models also grows. 
For instance, on the five stages from \textit{Arithmetic} to \textit{College} Math, 
it outperforms ChatGLM3-6B by 52.7\%, 66.7\%, 113.7\%, 376.6\%, and 1160.0\%, respectively. 
The trend indicates that as the difficulty escalates, the performance disparity between models significantly increases since higher-stage math problems often involve more complex concepts and problem-solving strategies, imposing greater demands on the models' comprehension and reasoning abilities. 
All $\sim$7B models struggle with advanced mathematical problems, 
% with InternLM2-Chat-7B achieving only 29.6\% and 22.6\% accuracies in High school and College math, respectively, 
indicating a challenge in smoothly resolving complex questions for small-scale LLMs.

\noindent \textbf{$\sim$20B Chat Models. }
InternLM2-Chat-20B performs the best at the $\sim$20B scale, followed by Qwen-14B-Chat. 
Though Yi-34B-Chat has a much larger parameter size, 
it lags behind other $\sim$20B models. 
Similar to $\sim$7B models, models around $\sim$20B also struggle with more complex mathematical problems at the \textit{High School} and \textit{College} stage.

\noindent \textbf{$\sim$70B Chat Models and Math Models. }
In the realm of large-scale open-source language models, a significant performance disparity is evident when comparing models of varying sizes. Notably, the Qwen-72B-Chat model has shown exceptional proficiency in addressing mathematical application problems. Its performance not only surpasses that of other open-source chat-oriented models but also eclipses the capabilities of numerous specialized mathematical models.

Focusing on models dedicated to mathematical tasks, the DeepSeek-Math-7B-RL model stands out for its adeptness in tackling application-based questions across a spectrum of stages, encompassing basic \textit{Primary}, \textit{High} and \textit{College} math. Remarkably, it outstrips not only its counterparts, but also the substantially larger DeepSeek-67B-Chat model, by a margin of 22.7\%. This is particularly noteworthy given that the DeepSeek-Math-7B-RL achieves this superior performance with a model size nearly one-tenth that of the DeepSeek-67B-Chat, underscoring the efficiency and targeted capability of the former in mathematical problem-solving domains.

%Qwen-72B-Chat, for instance, achieves excellent results across all stages, which is comparable to the state-of-the-art GPT-4.%
% ADD



\subsubsection{MathBench-T}

In the theoretical part of MathBench, referred to as MathBench-T, GPT-4 consistently achieved balanced and excellent results across all theoretical stages, achieving an average theoretical score of 78.6. This score was the best among all tested Closed-source Models and Open-source Chat Models. Combined with an application score of 55.6 in MathBench-A, it demonstrates that GPT-4 has balanced and superior performance in both theory and application on MathBench. This proves that it not only has a good grasp of theoretical knowledge but also excels in the application of such knowledge.

Among other models except GPT-4, the Qwen series models stood out, with Qwen-Max and Qwen-72B-Chat ranking just behind GPT-4. Notably, in the theoretical stage of \textit{Primary}, Qwen-72B-Chat scored the highest among all models with an 89.4 CE score. However, GPT-4's advantage lies in higher educational stages or perhaps more advanced theoretical stages. For example, in the college-level theoretical knowledge stage, GPT-4 scored a 79.8 CE score, which is 11.8 points higher than the best open-source model, Deepseek-Math-7B-RL.

Similar to MathBench-A, InternLM2-Chat-7B showed strong theoretical capabilities at the common models of 7B stage, but it had an even larger lead in the theoretical stage, leading by 34.4\% compared to the next best model, Qwen-7B-Chat. In the realm of mathematical chat models, Deepseek-Math-7B-RL still surpassed a host of mathematical models, achieving the best results in both theory and application, even showing similar performance to the Closed-source Model Claude-3-Opus.

Overall, in the tests conducted on MathBench, there was not a significant rank change between models in terms of theoretical and application capabilities. That is, models that ranked highly in application capabilities also tended to perform well in theoretical tests, and vice versa.


% This performance highlights DeepSeek-Math-7B-RL's robust mathematical capabilities, spanning from basic \emph{arithmetic} to complex \emph{college}-stage mathematical challenges, despite having a smaller model size.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figs/application_average.png}
    \caption{\textbf{Scores of Application Problems at Each Stage}. 
    Models exhibit similar performances in \emph{Arithmetic} and \emph{Primary} stages, while demonstrating a clear performance decline from \emph{Primary} to \emph{College} stages.}
    \label{fig:application_average}
\end{figure}


\subsection{Evaluation of Base Models}
\input{tabs/application_theory_base_tab}
The results for the Base models are presented in \Cref{tab: application_theory_base_result}. Consistency in performance is observed between the Base models and their Chat model counterparts, with InternLM2-7B emerging as the optimal model in the 7B parameter range. Qwen-14B and Qwen-72B demonstrate superior performance within their respective parameter classes on the MathBench benchmark. For mathematical tasks, Deepseek-Math-7B-Base's results align closely with those seen in the Chat model evaluations, indicating a significant correlation between the efficacy of Base models and their corresponding Chat models, which leads to similar performance trends across models within the same category.

Notably, ChatGLM3-6B-Base secures the second-highest ranking in the 7B base model evaluation, outperforming several other models, including Qwen-7B and Mistral-7B-v0.1. However, this performance is not mirrored in its Chat model variant, ChatGLM3-6B, which is surpassed by Qwen-7B-Chat by 95.2\% on MathBench-A and by 104.7\% on MathBench-T. This discrepancy in performance between the Chat and Base versions of the model may be attributed to the different fine-tuning strategies applied during the subsequent tuning phase, which could explain the observed gap in performance.


\subsection{Detailed Analysis}
% 在MathBench预定义的体系框架内，我们可以轻易的测的模型关于数学能力的各种信息，不仅可以精确到学段和语言，甚至可以精确到具体的知识点下的应用题和知识题的问答情况，图 \ref{practice_average} 代表了上述模型在数学应用题的整体梯度结果，可见大多数模型都在四则运算和小学难度数学题目上有着还不错的表现，对于初中及以上的题目效果就急剧地成梯度式下降
With MathBench, 
we can easily assess the model's mathematical capabilities at different granularities including education stage, language, subject area, or even specific topics with questions on both theories and applications.
Below, we will delve deeper into the evaluation results and discuss about the following questions: 

\paragraph{The Gap between Circular and Accuracy Evaluation}
A comparison between Circular Evaluation (CE) scores and Accuracy (ACC) scores is illustrated in \Cref{fig:acc ce comparison}. As model performance improves, the discrepancy between CE and ACC scores becomes increasingly narrow, suggesting that more powerful models tend to provide more robust and stable answers in mathematical question answering.

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figs/acc_ce_comparison.png}
    \caption{\textbf{CE Evaluation vs. ACC Evaluation}. The ACC evaluation queries the model once per question and checks for correctness, whereas the CE (CircularEval) conducts a more stringent and robust assessment by rolling out evaluations four times with shuffled answer options, deeming a question correct only if all attempts are accurate. The percentages depicted in the figure represent the performance decrease of models in the CE evaluation compared to the ACC evaluation.}
    \label{fig:acc ce comparison}
\end{figure*}

\begin{figure}[!ht]
\centering
\includegraphics[width=1\linewidth]{figs/bilingual.png}
\caption{\textbf{Bilingual Comparison on MathBench}. showcasing scores in Chinese, English , and their average for the gray dashed line. The \textit{Arithmetic} stage is not include because there no impact of language in it.}
\label{fig:bilingual-ability}
\end{figure}


\paragraph{How Models' Scores on Application Problems Vary Across Stages?}
Figure \ref{fig:application_average} presents the average performance of all aforementioned models on application questions in MathBench. 
Most models perform reasonably well on \textit{Arithmetic} and \textit{Primary} math problems. 
However, their effectiveness drastically declines when it comes to the \textit{Middle} stage or above. 
% while models are becoming increasingly proficient at handling basic arithmetic and primary school problems, there is a marked performance gap at higher levels of mathematical complexity. 
Such phenomenon suggests that existing models are good at tasks that can be solved through direct computation, pattern recognition, or memorizing basic concepts.
However, they showcase inferior performance when solving more complex math problems. 


\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figs/app_theory_with_stages.png}
    \caption{\textbf{Theoretical Score vs. Applied Score on MathBench}. \textit{Primary} and \textit{Arithmetic} are averaged because they share the same theory knowledge points.}
    \label{fig:app_theory_with_stages}
\end{figure*}


\paragraph{Is There A Gap between Theory Understanding and Application Capabilities?} 
% Figure \ref{fig:app_theory_with_stages} presents a scatter plot of the average scores for theoretical and application questions achieved by selected representative models. To more accurately reflect the models' tendencies towards theoretical and practical abilities on MathBench, we display the scores after standardizing them. As shown in the figure, most of the representative models achieve a balance between theoretical and practical mathematical problem-solving. Specifically, the Qwen series models, Qwen-7B-Chat, Qwen-14B-Chat, and Qwen-72B-Chat, exhibit a similar trend, slightly favoring theoretical aspects.

% In contrast, GPT-4 performs well in both theoretical and practical capabilities, with a stronger inclination towards solving practical problems like InternLM2-Chat-7B. GPT-3.5 and DeepSeek-Math-7B-RL are more balanced in their performance. It is worth noting that, from a theoretical perspective, the theoretical capabilities of Qwen-72B-Chat and DeepSeek-Math-7B-RL are not significantly different from GPT-4. However, there is a noticeable gap in their mathematical application abilities, indicating that the GPT-4 model is better at applying theoretical knowledge to solve practical problems based on its mastery of theory.Detailed data can be found in Appendix Table. \ref{tab: practice_theory_result}.

Theories serve as the foundation for addressing the majority of application problems. 
As illustrated in \Cref{fig:app_theory_with_stages}, 
we present the trend of LLMs in terms of theoretical and application scores across different stages. 
In the \textit{Primary} stage, the two scores are highly correlated for most LLMs, with only a few exceptions. 
% Metamath-Llemma-7B exhibits a significant gap in theoretical ability compared to its application ability, which is comparable to that of Qwen-7B-Chat and Baichuan2-13B-Chat. 
Among top-ranked models, Qwen-72B-Chat demonstrates the best theoretical ability, while Claude-3-Opus demonstrates superior application ability. 
When it comes to more advanced stages, 
models require better computational and reasoning capabilities to achieve good application scores. 
GPT-4 leads in the application track across all stages,
while the gap is larger in more advanced stages. 
For example, 
comparing to Qwen-72B-Chat,
the difference in theoretical and application scores $(D_t,D_a)$ increases from $(1.4, 8.7)$ in the \textit{Middle} stage to $(6.0, 11.7)$ in the \textit{High} stage, and finally to $(13.5, 23.0)$ in the \textit{College} stage. 
Moreover, from the \textit{Middle} stage onwards, there is a general trend of decline in both theoretical and application abilities of models. 
Compared to theoretical scores, the decline in application scores is more serious. 
% This implies that, assuming constant theoretical abilities, the decline in application abilities is more evident. 

% A detailed discussion on this trend can be found in  \Cref{app:trending_analysis}.

\begin{figure*}[!th]
    \centering
    \includegraphics[width=1\linewidth]{figs/average_topic.pdf}
    \caption{\textbf{Average Model Scores with Topics}. We average the scores of every Chat model for each topic in MathBench. The models excel at basic-level problems, such as single Unit Conversion and basic Four Operations, but as the required reasoning and computational abilities for a topic increase, the performance of the models gradually declines, as observed in topics like Double Integrals, Set Theory, and Mathematical Logic.}
    \label{fig:average topic}
\end{figure*}

\paragraph{Detailed Model Performance for Each Topic}
In \Cref{fig:average topic} indicating average knowledge point performance, it is evident that topics associated with fundamental mathematical skills—such as 'Unit Conversion,' 'Four Operations,' and 'Basic Concepts of Equations'—register higher average scores. This suggests that the majority of models exhibit a proficient command of simple and elementary mathematical questions.

Conversely, topics demanding abstract reasoning and intricate computations, like 'Double Integrals,' 'Mathematical Logic,' and 'Set Theory,' show lower average scores. Addressing the mathematical queries in these topics may require bespoke model analysis and optimization. It is crucial to pinpoint the source of inaccuracies within these topics, whether it be due to a deficit in reasoning ability or an unstable grasp of the relevant foundational theoretical concepts.

\paragraph{Which Model Performs Better under the Bilingual Scenario?}
\Cref{fig:bilingual-ability} demonstrates the bilingual capabilities of various LLMs on MathBench, indicating the importance of linguistic versatility in mathematical tasks that demand an understanding of nuances in language and math concepts across different languages.
Among all LLMs, GPT-4 leads with the highest bilingual score of 67.1, showing a balanced performance between Chinese (65.2) and English (69.0). This demonstrates GPT-4's advanced bilingual processing abilities.
% , making it a benchmark for bilingual language models and highlighting its potential to bridge linguistic divides on a global scale.
Other models including Qwen-72B-Chat and DeepSeek-Math-7B-RL also exhibit significant bilingual capabilities. 
It's also noteworthy that among all LLMs evaluated, most of them feature a much larger performance gap between Chinese and English, compared to GPT-4. The detailed result of bilingual test of MathBench can be found in \Cref{app: bilingual results}.
% though their performances indicate the challenges in achieving consistent proficiency across languages.
% For instance, Qwen-72B-Chat, with an average score of 58.4, shows a stronger performance in Chinese, pointing to potential variations in training data, model architecture, or fine-tuning strategies.
% DeepSeek-Math-7B-RL, with balanced scores of 54.9 in Chinese and 58.1 in English, suggests a strategy that might favor an equitable distribution of language-specific resources. This indicates the advantages of diverse training datasets that cover a wide range of linguistic and mathematical content.

\paragraph{Enhancing Model Proficiency in Fundamental Theories: Initial Explorations}
In an effort to augment the model's grasp and application of theoretical concepts in problem-solving contexts, we embarked on exploratory initiatives, focusing primarily on two methodologies: Chain of Thought (CoT) and Knowledge Infusion.

We selectively sampled 200 questions from MathBench, deliberately skewed towards theoretical reasoning and application (with a distribution of 40\% application-oriented and 60\% theory-centric questions), to perform ancillary experiments on the Qwen-72B-Chat model. The outcomes, delineated in Table~\ref{tab:enhance concept}, elucidate the accuracy achieved through different strategic approaches.

\begin{itemize}
    \item \textbf{Straight:} Immediate response without preceding CoT.
    \item \textbf{CoT:} Response derived post-CoT, serving as MathBench's standard evaluative criterion.
    \item \textbf{Straight-Knowledge:} Immediate response, preconditioned by the integration of relevant knowledge points prior to posing the question.
    \item \textbf{CoT-Knowledge:} Response post-CoT, facilitated by the preliminary inclusion of pertinent knowledge points.
\end{itemize}

\begin{table}[h!]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Strategy}           & \textbf{Accuracy (\%)} \\ \hline
Straight           & 26.6     \\ 
CoT                & 29.8     \\ 
Straight-Knowledge & 31.3     \\ 
CoT-Knowledge      & 33.4     \\ \hline
\end{tabular}
\caption{Comparative accuracy of different strategies.}
\label{tab:enhance concept}
\end{table}

Knowledge points were meticulously curated from academic textbooks and instructional resources. The experimental data suggests a progressive enhancement in efficacy: Straight < CoT < Straight-Knowledge < CoT-Knowledge. This progression evidences the significant impact of both CoT and knowledge point infusion on augmenting model performance for questions heavily reliant on theoretical reasoning or practical application, with their combined utilization yielding the most favorable outcomes.


\section{Discussion}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/scale_score.png}
     \caption{\textbf{Model Size vs. Average Score}. The comparison chart of model parameter size versus performance on MathBench for selected representative models, with models from the same series connected by lines of the same color. The horizontal red dotted line represents the score of GPT-4.} 
    \label{fig:scale_score}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figs/image.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

% ADD
\subsection{How Models Perform with Code Agent on MathBench}
We utilize the external code interpreter and follow the ReAct~\citep{yao2023react} protocol to evaluate LLMs' ability to solve coding and mathematic problems. The results, as depicted in \Cref{fig: code_agent_results}, show the comparison of performance with and without the Code Agent on the Theory and Application sections of MathBench. Overall, the inclusion of the Code Agent significantly enhances performance in the Application section, especially in Arithmetic, where it boosts the performance of InternLM2-7B-Chat by about 64\% (from 53.0 to 87.3). This demonstrates that the addition of the Code Agent can substantially improve the model's basic numerical calculation capabilities. However, for more complex problems, such as those in the College level Application section, the Code Agent does not notably improve model capabilities and even slightly degrades performance. For theoretical problems, the Code Agent does not significantly enhance InternLM2-7B-Chat's performance across various stages on MathBench. This suggests that mathematical theoretical ability, as a crucial foundational skill for models, requires more than just external tools. Instead, it necessitates exploring more effective ways to enhance large language models' understanding and application of mathematical concepts.

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figs/app_with_code.png}
        % \caption{Caption for the first image.}
        \label{fig:code_agent1}
    \end{subfigure}
    \hfill % This command adds space between the two figures
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figs/theory_with_code.png}
        % \caption{Caption for the second image.}
        \label{fig:code_agent2}
    \end{subfigure}
    \caption{\textbf{Code Agent Performance on MathBench}. We use InternLM2-7B-Chat for the comparison and the results are divided into two parts with stages: Application and Theory. }
    \label{fig: code_agent_results}
\end{figure*}


\subsection{Effect of Model Size on Math Capabilities}
We found that for models of different sizes within the same series, 
most of them conform to the Scaling Law~\citep{kaplan2020scaling} on MathBench.
For example, Qwen series, MammoTH series, and Yi series have shown steady improvement in their MathBench scores as the parameter size increases, 
as shown in \Cref{fig:scale_score}. 
However, it doesn't mean that models with small parameter sizes can not achieve good math performance.
For instance, DeepSeek-Math-7B demonstrates outstanding performance on MathBench and outperforms models with 10x parameters, including DeepSeek-72B and a larger math model MammoTH-70B. 
% This indicates that the mathematical ability may not have been fully exploited in terms of the number of parameters. 
% We can still look forward to the capabilities of smaller models, such as 2B or even smaller, in solving mathematical problems at various stages, especially with the adoption of newer training methods and high quality corpora~\citep{deepseekmath}.

\subsection{Error Analysis}
In our study, we conduct a comprehensive error analysis on a set of 80 theoretical and 100 application questions random selected from every stages, for models selected across different scales, as illustrated in \Cref{fig:response-error-analysis}. 
The error categories are uniformly observed across all evaluated models, indicating common challenges that transcend specific parameter scales.
Our selection of models includes GPT-3.5, GPT-4, InternLM2-Chat-7B, Qwen-14B-Chat, Qwen-72B-Chat, Deepseek-Math-7B-RL and MammoTH-70B. Detailed cases for error analysis can be found in \Cref{app: error analysis}.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/error.png}
    \caption{\textbf{Response Error Analysis for Both Theoretical and Application Questions. } The predominant sources of errors are a fundamental misunderstanding of the concepts, followed by incorrect reasoning paths.}
    \label{fig:response-error-analysis}
\end{figure}

%app:error_analysis为附录error相关的cases
%This investigation aimed to identify and categorize prevalent error types, which included misunderstandings of mathematical concepts, logically consistent yet flawed reasoning, reasoning misaligned with the query's intent, responses constrained to selections, and responses exceeding the predefined character limit. 

\noindent \textbf{Insufficiency of knowledge. } 
For theoretical questions, 78\% of model errors are due to misconceptions about mathematical concepts, 
which notably emerged as a significant concern in several models. 
Such errors accounted for 49.5\% of all mistakes, 
underscoring a general challenge in grasping fundamental knowledge and terminology.

\noindent \textbf{Deficiencies in reasoning. } 
Furthermore, models exhibited shortcomings in logical reasoning, with 33.4\% of errors attributed to logically consistent but flawed reasoning processes.
Moreover, errors such as reasoning that deviated from the intended query accounting for 9.6\%, underscored the models' limitations in understanding user intentions and providing pertinent responses. 
% [{\color{red} add }] 
We also notice that errors related to reasoning increased with task difficulty.

\noindent \textbf{Response length limit. } 
Though statistically not the primary error mode (4.0\%), 
responses that exceeded the token limit shed light on the challenge of reasoning complex tasks within limited length and adhering to given instructions.

\noindent \textbf{Other cases. } 
Occasionally, models will generate responses devoid of an explicit reasoning process, 
obstructing additional scrutiny. 
Moreover, models endowed with enhanced reasoning capabilities exhibit a greater capacity for critical thinking regarding the options presented, 
thereby offering alternative answers that transcend the limitations of predetermined choices.

% {\color{red} [split and moved to other paragraphs]}
% \hd{Difficult to understand, please refine this paragraph. }

\subsection{Reasoning Path}
Analyzing the reasoning paths of various models across multiple difficulty levels reveals significant performance disparities. 
We set a brief discussion below and provide more detailed cases for reasoning path analysis in \Cref{app: reasoning path}.

\noindent \textbf{Performance across diverse difficulties. } 
In straightforward scenarios, models swiftly solve the problems with direct reasoning and yield logical outcomes. 
Yet, complex issues, marked by dense symbols, vast knowledge, and intricate links, necessitate broader knowledge navigation, accentuating divergences in deductive strategies.

\noindent \textbf{Reasoning paths of chat models with different parameter sizes. } 
Small-scale chat models strive for logical coherence in mathematics, 
yet may make mistakes due to knowledge deficiencies, 
particularly in symbol interpretation and relational understanding. 
In contrast, large-scale models feature expansive knowledge and nuanced insights, which enhance symbol processing and minimizing knowledge gaps. 
However, even with substantial parameters, challenges in efficient knowledge  management persist, 
occasionally leading to irrelevant diversions and diminished reasoning efficacy.

\noindent \textbf{Reasoning paths of math models. } 
Specialized math models, despite the smaller parameter sizes, exhibit superior mathematical comprehension and systematic logical reasoning. 
% [{\color{red} refine}] 
They excel in applying mathematical knowledge and notation to reason through complex problems. 
% \hd{What is nagative complex tasks, is that usage proper? }

\noindent \textbf{Superlative deductive navigation of Closed-source models. } 
GPT-4 stands out for its effective reasoning and deep problem comprehension. 
It engages in logical, coherent, and succinct discussions, adeptly navigate complex reasoning paths, and manage mathematical symbols effectively. GPT-4 distinctively recognizes problem statement ambiguities, showcasing a detailed and nuanced reasoning process.

==> tabs/acc_results_512.tex <==
% \begin{table*}[!thb]
% \centering
% \caption{\textbf{Overall Comparison with Accuracy on MathBench}. Models are classified into three categories according to their purpose and origin. The model name in \textbf{bold} indicates the top performer among Open-Source or Closed-source models, while an \underline{underline} signifies the leading model within a similar parameter size group.}
% \vspace{-2mm}
% \label{tab:acc_results}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc|c}
% \hline
% \textbf{Models} & \textbf{Arithmetic} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Average} \\
% \hline
% \multicolumn{7}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
% GPT-3.5 & 70.3 & 67.9 & 52.6 & 46.4 & 46.6 & 56.8 \\
% GPT-4 & \textbf{76.3} & \textbf{82.9} & \textbf{76.8} & \textbf{66.8} & \textbf{70.4} & \textbf{74.6} \\
% \hline
% \multicolumn{7}{c}{\bluecolor{\textit{$\heartsuit$Open-Source Chat Models}}} \\
% ChatGLM3-6B & 41.0 & 40.5 & 36.3 & 23.3 & 17.2 & 31.7 \\
% Yi-6B-Chat & 35.7 & 41.1 & 33.2 & 22.4 & 20.2 & 30.5 \\
% InternLM2-Chat-7B & \underline{53.0} & \underline{67.5} & \underline{52.3} & \underline{39.4} & \underline{36.6} & \underline{49.8} \\
% Qwen-7B-Chat & 51.3 & 50.2 & 42.3 & 31.7 & 28.9 & 40.9 \\
% Deepseek-7B-Chat & 46.0 & 39.3 & 29.5 & 20.5 & 19.5 & 31.0 \\
% \hline
% Baichuan2-13B-Chat & 46.0 & 54.2 & 42.6 & 27.5 & 24.0 & 38.9 \\
% Qwen-14B-Chat & \underline{64.7} & 48.2 & \underline{60.3} & \underline{45.8} & \underline{40.6} & 52.0 \\
% InternLM2-Chat-20B & 62.7 & \underline{70.0} & 57.1 & 44.2 & 34.1 & \underline{53.6} \\
% Yi-34B-Chat & 51.0 & 64.8 & 49.4 & 32.2 & 28.0 & 45.1 \\
% \hline
% DeepSeek-67B-Chat & 61.3 & 77.2 & 60.2 & 46.4 & 47.5 & 58.5 \\
% Qwen-72B-Chat & \textbf{72.0} & \underline{80.0} & \textbf{74.0} & \textbf{59.8} & \textbf{52.8} & \textbf{67.7}} \\
% \hline
% \multicolumn{7}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
% Mammoth-7B & 26.7 & 18.1 & 14.5 & 14.3 & 15.2 & 17.7 \\
% Metamath-Llemma-7B & 48.7 & 35.3 & 26.3 & 24.5 & 19.2 & 30.8 \\
% InternLM2-Chat-Math-7B & 53.7 & 67.4 & 60.5 & 49.7 & 42.8 & 54.8 \\
% DeepSeek-Math-7B-Instruct & 61.0 & 73.7 & 53.0 & 47.7 & 44.4 & 56.0 \\
% DeepSeek-Math-7B-RL & \underline{67.7} & \underline{\textbf{80.8} & \underline{64.4} & \underline{54.8} & \underline{42.3} & \underline{62.0} \\
% Mammoth-13B & 35.0 & 34.8 & 22.2 & 20.7 & 22.2 & 27.0 \\
% InternLM2-Chat-Math-20B & 58.7 & 69.6 & 63.3 & 52.3 & 42.8 & 57.3 \\
% Mammoth-70B & 35.7 & 59.3 & 41.3 & 33.3 & 35.5 & 41.0 \\

% \hline
% \end{tabular}}
% \end{table*}


\begin{table*}[!thb]
\centering
\caption{\textbf{Overall Comparison with Accuracy on MathBench}. Models are classified into three categories according to their purpose and origin. The model name in \textbf{bold} indicates the top performer among Open-source or Closed-source models, while an \underline{underline} signifies the leading model within a similar parameter size group.}
\vspace{-2mm}
\label{tab:acc_results_512}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc|c}
\hline
\textbf{Models} & \textbf{Arithmetic} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Average} \\
\hline
\multicolumn{7}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 70.3 & 76.8 & 63.8 & 59.3 & 60.3 & 66.1 \\
GLM4 & 61.3 & 86.4 & 80.9 & 71.9 & 64.6 & 73.0 \\
Qwen-Max & 69.3 & 87.0 & 79.6 & 71.9 & 68.3 & 75.2 \\
Claude-3-Opus & \textbf{84.7} & \textbf{88.8} & 80.2 & 69.6 & 63.6 & 77.4 \\
GPT-4 & 76.3 & 85.7 & \textbf{81.2} & \textbf{74.6} & \textbf{76.1} & \textbf{78.8} \\
\hline
\multicolumn{7}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
Yi-6B-Chat & 35.7 & 51.7 & 49.5 & 38.1 & 37.5 & 42.5 \\
Deepseek-7B-Chat & 46.0 & 54.8 & 43.6 & 36.3 & 36.6 & 43.5 \\
ChatGLM3-6B & 41.0 & 53.2 & 51.2 & 38.9 & 34.0 & 43.7 \\
InternLM2-Chat-7B & \underline{53.0} & \underline{75.9} & \underline{63.7} & \underline{52.6} & \underline{51.1} & \underline{59.3} \\
\hline
Baichuan2-13B-Chat & 46.0 & 64.4 & 54.8 & 42.1 & 40.3 & 49.5 \\
Qwen-7B-Chat & 51.3 & 63.4 & 55.4 & 45.4 & 43.5 & 51.8 \\
Yi-34B-Chat & 51.0 & 74.1 & 61.2 & 46.2 & 42.1 & 54.9 \\
Qwen-14B-Chat & \underline{64.7} & 75.1 & \underline{69.6} & \underline{58.8} & \underline{52.4} & 64.1 \\
InternLM2-Chat-20B & 62.7 & \textbf{81.8} & 68.6 & 58.2 & 52.3 & \underline{64.7} \\
\hline
DeepSeek-67B-Chat & 61.3 & \underline{83.2} & 68.5 & 56.5 & 56.9 & 65.3 \\
Qwen-72B-Chat & \textbf{72.0} & 81.7 & \textbf{78.8} & \textbf{68.2} & \textbf{60.4} & \textbf{72.2} \\
\hline
\multicolumn{7}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
Mammoth-7B & 26.7 & 30.8 & 30.7 & 25.7 & 28.6 & 28.5 \\
Metamath-Llemma-7B & 48.7 & 45.4 & 36.5 & 34.8 & 31.8 & 39.4 \\
InternLM2-Chat-Math-7B & 53.7 & 77.9 & \underline{72.5} & 61.1 & 54.9 & 64.0 \\
DeepSeek-Math-7B-Instruct & 61.0 & 80.1 & 62.7 & 59.1 & 57.1 & 64.0 \\
DeepSeek-Math-7B-RL & \underline{67.7} & \textbf{86.0} & 70.6 & \underline{64.2} & \underline{59.4} & \underline{69.6} \\
Mammoth-13B & 35.0 & 47.8 & 38.3 & 36.6 & 37.1 & 39.0 \\
InternLM2-Chat-Math-20B & 58.7 & 77.9 & 73.0 & 62.3 & 54.9 & 65.4 \\
Mammoth-70B & 35.7 & 68.7 & 53.1 & 45.4 & 46.5 & 49.9 \\
\hline
\end{tabular}}
\end{table*}



==> tabs/application_tab.tex <==
\begin{table*}[!thb]
\centering
\caption{\textbf{Overall Comparison of Models on MathBench-A}. We present scores for application questions here. Models are classified into three categories according to their purpose and origin. The model name in \textbf{bold} indicates the top performer among Open-source or Closed-source models, while an \underline{underline} signifies the leading model within a similar parameter size group.}
\label{tab: application_result}
\begin{tabular}{lccccc|c}
\hline
\textbf{Models} & \textbf{Arithmetic} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Average} \\
\hline
\multicolumn{7}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 70.3 & 69.0 & 27.7 & 17.3 & 17.0 & 32.8 \\
Qwen-Max & 69.3 & 80.7 & 50.3 & 33.7 & 20.7 & 46.4 \\
GLM4 & 61.3 & 79.0 & 54.0 & 41.3 & 21.0 & 48.8 \\
Claude-3-Opus & \textbf{84.7} & \textbf{85.3} & 54.0 & 33.3 & 24.0 & 49.1 \\
GPT-4 & 76.3 & 80.3 & \textbf{61.3} & \textbf{42.3} & \textbf{38.3} & \textbf{55.6} \\
\hline
\multicolumn{7}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
Yi-6B-Chat & 35.7 & 36.0 & 7.3 & 3.7 & 1.3 & 12.1 \\
Deepseek-7B-Chat & 46.0 & 45.7 & 5.0 & 3.7 & 1.8 & 14.0 \\
ChatGLM3-6B & 41.0 & 42.7 & 11.7 & 3.0 & 0.5 & 14.5 \\
Qwen-7B-Chat & 51.3 & 48.7 & 22.0 & 9.7 & 5.5 & 21.5 \\
InternLM2-Chat-7B & \underline{53.7} & \underline{67.7} & \underline{25.0} & \underline{14.3} & \underline{6.3} & \underline{28.3} \\
\hline
Baichuan2-13B-Chat & 46.0 & 50.3 & 14.7 & 3.3 & 3.7 & 18.0 \\
Yi-34B-Chat & 51.0 & 60.3 & 23.7 & 7.3 & 2.7 & 23.5 \\
Qwen-14B-Chat & 64.7 & 61.3 & 36.7 & 19.7 & 7.8 & 31.4 \\
InternLM2-Chat-20B & \underline{62.7} & \underline{75.7} & \underline{39.7} & \underline{23.7} & \underline{13.7} & \underline{38.2} \\
\hline
Deepseek-67B-Chat & 61.3 & \underline{72.6} & 33.0 & 19.0 & 12.7 & 34.3 \\
Qwen-72B-Chat & \textbf{72.0} & 71.0 & \textbf{52.7} & \underline{30.7} & \underline{15.3} & \underline{42.4} \\
\hline
\multicolumn{7}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
MammoTH-7B & 26.7 & 24.3 & 3.0 & 1.3 & 1.0 & 7.4 \\
MammoTH-13B & 35.0 & 41.7 & 5.0 & 4.0 & 4.3 & 13.8 \\
Metamath-Llemma-7B & 48.7 & 49.3 & 9.0 & 9.0 & 4.0 & 17.8 \\
MammoTH-70B & 35.7 & 60.7 & 11.0 & 8.3 & 5.3 & 21.3 \\
InternLM2-Chat-Math-7B & 58.7 & 67.0 & 40.3 & 18.0 & 7.3 & 33.2 \\
Deepseek-Math-7B-Instruct & 61.0 & 74.0 & 29.7 & 21.3 & 9.7 & 33.7 \\
InternLM2-Chat-Math-20B & 53.7 & 70.0 & 43.0 & 24.3 & 11.3 & 37.2 \\
Deepseek-Math-7B-RL & \underline{67.7} & \textbf{82.7} & \underline{44.7} & \textbf{31.0} & \textbf{17.3} & \textbf{43.9} \\
\hline
\end{tabular}
\end{table*}

==> tabs/application_theory_tab.tex <==
% \begin{table*}[!htb]
%     \captionsetup{justification=centering}
%     \begin{minipage}{.55\linewidth}
%       \centering
%         \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc|c}
% \hline
% \textbf{Models} & \textbf{Arithmetic} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Average} \\
% \hline
% \multicolumn{7}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
% GPT-3.5 & 70.3 & 69.0 & 27.7 & 17.3 & 17.0 & 32.8 \\
% Qwen-Max & 69.3 & 80.7 & 50.3 & 33.7 & 20.7 & 46.4 \\
% GLM4 & 61.3 & 79.0 & 54.0 & 41.3 & 21.0 & 48.8 \\
% Claude-3-Opus & \textbf{84.7} & \textbf{85.3} & 54.0 & 33.3 & 24.0 & 49.1 \\
% GPT-4 & 76.3 & 80.3 & \textbf{61.3} & \textbf{42.3} & \textbf{38.3} & \textbf{55.6} \\
% \hline
% \multicolumn{7}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
% Yi-6B-Chat & 35.7 & 36.0 & 7.3 & 3.7 & 1.3 & 12.1 \\
% Deepseek-7B-Chat & 46.0 & 45.7 & 5.0 & 3.7 & 1.8 & 14.0 \\
% ChatGLM3-6B & 41.0 & 42.7 & 11.7 & 3.0 & 0.5 & 14.5 \\
% Qwen-7B-Chat & 51.3 & 48.7 & 22.0 & 9.7 & 5.5 & 21.5 \\
% InternLM2-Chat-7B & \underline{53.7} & \underline{67.7} & \underline{25.0} & \underline{14.3} & \underline{6.3} & \underline{28.3} \\
% \hline
% Baichuan2-13B-Chat & 46.0 & 50.3 & 14.7 & 3.3 & 3.7 & 18.0 \\
% Yi-34B-Chat & 51.0 & 60.3 & 23.7 & 7.3 & 2.7 & 23.5 \\
% Qwen-14B-Chat & 64.7 & 61.3 & 36.7 & 19.7 & 7.8 & 31.4 \\
% InternLM2-Chat-20B & \underline{62.7} & \underline{75.7} & \underline{39.7} & \underline{23.7} & \underline{13.7} & \underline{38.2} \\
% \hline
% Deepseek-67B-Chat & 61.3 & \underline{72.6} & 33.0 & 19.0 & 12.7 & 34.3 \\
% Qwen-72B-Chat & \textbf{72.0} & 71.0 & \textbf{52.7} & \underline{30.7} & \underline{15.3} & \underline{42.4} \\
% \hline
% \multicolumn{7}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
% MammoTH-7B & 26.7 & 24.3 & 3.0 & 1.3 & 1.0 & 7.4 \\
% MammoTH-13B & 35.0 & 41.7 & 5.0 & 4.0 & 4.3 & 13.8 \\
% Metamath-Llemma-7B & 48.7 & 49.3 & 9.0 & 9.0 & 4.0 & 17.8 \\
% MammoTH-70B & 35.7 & 60.7 & 11.0 & 8.3 & 5.3 & 21.3 \\
% InternLM2-Chat-Math-7B & 58.7 & 67.0 & 40.3 & 18.0 & 7.3 & 33.2 \\
% Deepseek-Math-7B-Instruct & 61.0 & 74.0 & 29.7 & 21.3 & 9.7 & 33.7 \\
% InternLM2-Chat-Math-20B & 53.7 & 70.0 & 43.0 & 24.3 & 11.3 & 37.2 \\
% Deepseek-Math-7B-RL & \underline{67.7} & \textbf{82.7} & \underline{44.7} & \textbf{31.0} & \textbf{17.3} & \textbf{43.9} \\
% \hline
% \end{tabular}
%         }
%         \caption*{\small{MathBench-A.}}
%     \end{minipage}%
%     \begin{minipage}{.47\linewidth}
%       \centering
        
%         \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccc|c}
% \hline
% \textbf{Models} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Average} \\
% \hline
% \multicolumn{6}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
% GPT-3.5 & 66.8 & 50.9 & 43.8 & 47.5 & 52.3 \\
% Claude-3-Opus & 87.0 & 73.0 & 63.1 & 53.3 & 69.1 \\
% GLM4 & 87.0 & 74.0 & 62.8 & 61.4 & 71.3 \\
% Qwen-Max & \textbf{87.8} & 75.0 & 69.0 & 73.3 & 76.3 \\
% GPT-4 & 85.4 & \textbf{78.3} & \textbf{70.9} & \textbf{79.8} & \textbf{78.6} \\
% \hline
% \multicolumn{6}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
% Deepseek-7B-Chat & 33.0 & 26.0 & 15.4 & 16.6 & 22.8 \\
% ChatGLM3-6B & 38.4 & 31.2 & 20.0 & 12.0 & 25.4 \\
% Yi-6B-Chat & 46.2 & 33.3 & 19.4 & 16.8 & 28.9 \\
% Qwen-7B-Chat & 51.7 & 43.3 & 30.7 & 29.1 & 38.7 \\
% InternLM2-Chat-7B & \underline{67.3} & \underline{57.0} & \underline{44.9} & \underline{38.8} & \underline{52.0} \\
% \hline
% Baichuan2-13B-Chat & 58.1 & 44.3 & 29.9 & 25.0 & 39.3 \\
% InternLM2-Chat-20B & 64.3 & 55.2 & 43.8 & 32.9 & 49.1 \\
% Yi-34B-Chat & 69.3 & 52.2 & 39.0 & 32.9 & 48.4 \\
% Qwen-14B-Chat & \underline{70.9} & \underline{61.8} & \underline{45.9} & \underline{46.5} & \underline{56.3} \\
% \hline
% Deepseek-67B-Chat & 78.1 & 63.8 & 53.5 & 60.9 & 64.1 \\
% Qwen-72B-Chat & \textbf{89.4} & \textbf{76.9} & \textbf{64.9} & \underline{66.3} & \textbf{74.4} \\
% \hline
% \multicolumn{6}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
% MammoTH-7B & 11.8 & 7.6 & 8.3 & 6.3 & 8.5 \\
% MammoTH-13B & 27.9 & 16.4 & 15.7 & 16.8 & 19.2 \\
% Metamath-Llemma-7B & 21.2 & 23.3 & 22.0 & 16.1 & 20.7 \\
% MammoTH-70B & 57.9 & 45.2 & 38.9 & 43.7 & 46.4 \\
% InternLM2-Chat-Math-7B & 64.9 & 57.7 & 50.7 & 46.5 & 55.0 \\
% Deepseek-Math-7B-Instruct & 73.3 & 54.7 & 48.5 & 50.2 & 56.7 \\
% InternLM2-Chat-Math-20B & 72.2 & 68.0 & 59.4 & 52.5 & 63.0 \\
% Deepseek-Math-7B-RL & \underline{78.9} & \underline{69.7} & \underline{59.9} & \textbf{68.0} & \underline{69.1} \\
% \hline
% \end{tabular}
%         }
%         \caption*{\small{MathBench-T.}}
%     \end{minipage}
%         \caption{\textbf{Overall Comparison of Models on MathBench-A \& T}. The \textit{Arithmetic} and \textit{Primary} stage for MathBench-T are combined because they share the same theory knowledge. Models are classified into three categories according to their purpose and origin. The model name in \textbf{bold} indicates the top performer among Open-source or Closed-source models, while an \underline{underline} signifies the leading model within a similar parameter size group.}
%     \label{tab: apllication_theory_chat_result}
% \end{table*}


\begin{table*}[!htb]
    % \captionsetup{justification=centering}
    \begin{minipage}{.52\linewidth}
      \centering
        \resizebox{\linewidth}{!}{
\begin{tabular}{lccccc|c}
\hline
\textbf{Models} & \textbf{Arith} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Avg.} \\
\hline
\multicolumn{7}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 70.3 & 69.0 & 27.7 & 17.3 & 17.0 & 40.3 \\
Qwen-Max & 69.3 & 80.7 & 50.3 & 33.7 & 20.7 & 50.9 \\
GLM4 & 61.3 & 79.0 & 54.0 & 41.3 & 21.0 & 51.3 \\
Claude-3-Opus & \textbf{84.7} & \textbf{85.3} & 54.0 & 33.3 & 24.0 & 56.3 \\
DeepSeek-V2 & 83.3 & 91.0 & 56.3 & 41.3 & 29.7 & 60.3 \\
GPT-4 & 76.3 & 80.3 & \textbf{61.3} & \textbf{42.3} & \textbf{38.3} & \textbf{59.7} \\

\hline
\multicolumn{7}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
Yi-6B-Chat & 35.7 & 36.0 & 7.3 & 3.7 & 1.3 & 16.8 \\
ChatGLM3-6B & 41.0 & 42.7 & 11.7 & 3.0 & 0.5 & 19.8 \\
Deepseek-7B-Chat & 46.0 & 45.7 & 5.0 & 3.7 & 1.8 & 20.4 \\
Qwen-7B-Chat & 51.3 & 48.7 & 22.0 & 9.7 & 5.5 & 27.4 \\
InternLM2-Chat-7B & \underline{53.7} & \underline{67.7} & \underline{25.0} & \underline{14.3} & \underline{6.3} & \underline{33.4} \\
\hline
Baichuan2-13B-Chat & 46.0 & 50.3 & 14.7 & 3.3 & 3.7 & 23.6 \\
Yi-34B-Chat & 51.0 & 60.3 & 23.7 & 7.3 & 2.7 & 29.0 \\
Qwen-14B-Chat & \underline{64.0} & 61.3 & 36.7 & 19.7 & 7.8 & 38.0 \\
InternLM2-Chat-20B & 62.7 & \underline{75.7} & \underline{39.7} & \underline{23.7} & \underline{13.7} & \underline{43.1} \\
\hline
Deepseek-67B-Chat & 61.3 & 72.6 & 33.0 & 19.0 & 12.7 & 39.7 \\
Qwen-72B-Chat & 72.0 & 71.0 & 52.7 & 30.7 & 15.3 & 48.3 \\
Qwen-1.5-110B-Chat & \textbf{72.3} & \textbf{83.7} & \textbf{62.0} & \textbf{41.3} & \textbf{18.7} & \textbf{55.6} \\
\hline
\multicolumn{7}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
MammoTH-7B & 26.7 & 24.3 & 3.0 & 1.3 & 1.0 & 11.3 \\
MammoTH-13B & 35.0 & 41.7 & 5.0 & 4.0 & 4.3 & 18.0 \\
Metamath-Llemma-7B & 48.7 & 49.3 & 9.0 & 9.0 & 4.0 & 24.0 \\
MammoTH-70B & 35.7 & 60.7 & 11.0 & 8.3 & 5.3 & 24.2 \\
InternLM2-Chat-Math-7B & 58.7 & 67.0 & 40.3 & 18.0 & 7.3 & 38.3 \\
Deepseek-Math-7B-Instruct & 61.0 & 74.0 & 29.7 & 21.3 & 9.7 & 39.1 \\
InternLM2-Chat-Math-20B & 53.7 & 70.0 & 43.0 & 24.3 & 11.3 & 40.5 \\
Deepseek-Math-7B-RL & \underline{67.7} & \underline{82.7} & \underline{44.7} & \textbf{31.0} & \textbf{17.3} & \textbf{48.7} \\
\hline
\end{tabular}
        }
        \caption*{\small{MathBench-A.}}
    \end{minipage}%
    \hfill
    \begin{minipage}{.47\linewidth}
      \centering
        
        \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc|c}
\hline
\textbf{Models} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Avg.} \\
\hline
\multicolumn{6}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 66.8 & 50.9 & 43.8 & 47.5 & 52.3 \\
Claude-3-Opus & 87.0 & 73.0 & 63.1 & 53.3 & 69.1 \\
GLM4 & 87.0 & 74.0 & 62.8 & 61.4 & 71.3 \\
Qwen-Max & \textbf{87.8} & 75.0 & 69.0 & 73.3 & 76.3 \\
DeepSeek-V2 & 88.7 & 82.7 & 68.9 & 76.3 & 79.1 \\
GPT-4 & 85.4 & \textbf{78.3} & \textbf{70.9} & \textbf{79.8} & \textbf{78.6} \\
\hline
\multicolumn{6}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
Deepseek-7B-Chat & 33.0 & 26.0 & 15.4 & 16.6 & 22.8 \\
ChatGLM3-6B & 38.4 & 31.2 & 20.0 & 12.0 & 25.4 \\
Yi-6B-Chat & 46.2 & 33.3 & 19.4 & 16.8 & 28.9 \\
Qwen-7B-Chat & 51.7 & 43.3 & 30.7 & 29.1 & 38.7 \\
InternLM2-Chat-7B & \underline{67.3} & \underline{57.0} & \underline{44.9} & \underline{38.8} & \underline{52.0} \\
\hline
Baichuan2-13B-Chat & 58.1 & 44.3 & 29.9 & 25.0 & 39.3 \\
InternLM2-Chat-20B & 64.3 & 55.2 & 43.8 & 32.9 & 49.1 \\
Yi-34B-Chat & 69.3 & 52.2 & 39.0 & 32.9 & 48.4 \\
Qwen-14B-Chat & \underline{70.9} & \underline{61.8} & \underline{45.9} & \underline{46.5} & \underline{56.3} \\
\hline
Deepseek-67B-Chat & 78.1 & 63.8 & 53.5 & 60.9 & 64.1 \\
Qwen-72B-Chat & \textbf{89.4} & \textbf{76.9} & \textbf{64.9} & \underline{66.3} & \textbf{74.4} \\
Qwen-1.5-110B-Chat & 92.0 & 82.7 & 81.7 & 80.9 & 84.3 \\
\hline
\multicolumn{6}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
MammoTH-7B & 11.8 & 7.6 & 8.3 & 6.3 & 8.5 \\
MammoTH-13B & 27.9 & 16.4 & 15.7 & 16.8 & 19.2 \\
Metamath-Llemma-7B & 21.2 & 23.3 & 22.0 & 16.1 & 20.7 \\
MammoTH-70B & 57.9 & 45.2 & 38.9 & 43.7 & 46.4 \\
InternLM2-Chat-Math-7B & 64.9 & 57.7 & 50.7 & 46.5 & 55.0 \\
Deepseek-Math-7B-Instruct & 73.3 & 54.7 & 48.5 & 50.2 & 56.7 \\
InternLM2-Chat-Math-20B & 72.2 & 68.0 & 59.4 & 52.5 & 63.0 \\
Deepseek-Math-7B-RL & \underline{78.9} & \underline{69.7} & \underline{59.9} & \textbf{68.0} & \underline{69.1} \\
\hline
\end{tabular}
        }
        \caption*{\small{MathBench-T.}}
    \end{minipage}
        \caption{\textbf{Overall Comparison of Models on MathBench-A \& T with Max Output Length Set to 512}. The \textit{Arithmetic} and \textit{Primary} stage for MathBench-T are combined because they share the same theory knowledge. Models are classified into three categories according to their purpose and origin. The model name in \textbf{bold} indicates the top performer among Open-source or Closed-source models, while an \underline{underline} signifies the leading model within a similar parameter size group.}
    \label{tab: apllication_theory_chat_result_max_out_512}
\end{table*}

==> tabs/bilingual.tex <==

\begin{table*}[!thb]
\centering
\caption{Detailed Results of Bilingual Score on MathBench (EN/CN).}
\label{tab: bilingual score}
\begin{tabular}{lcccc}
\hline
\textbf{Models} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} \\
\hline
\multicolumn{5}{c}{\textit{\purplecolor{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 76.5/59.3 & 39.2/25.3 & 41.7/33.4 & 42.9/21.5 \\
GPT-4 & 79.1/86.6 & 67.3/52.3 & 66.1/67.2 & 63.4/54.7 \\
\hline
\multicolumn{5}{c}{\textit{\bluecolor{$\heartsuit$Open-source Chat Models}}} \\
ChatGLM3-6B & 44.4/36.7 & 19.7/13.8 & 16.4/15.9 & 6.2/6.3 \\
Yi-6B-Chat & 42.9/39.2 & 19.5/17.5 & 13.0/13.7 & 9.6/8.5 \\
InternLM2-Chat-7B & 67.4/67.5 & 36.2/32.5 & 36.2/36.4 & 29.6/15.5 \\
Qwen-7B-Chat & 48.9/51.4 & 24.8/26.2 & 22.8/32.0 & 19.5/15.1 \\
Deepseek-7B-Chat & 43.4/35.2 & 16.3/11.7 & 12.9/9.2 & 9.7/8.7 \\
\hline
Baichuan2-13B-Chat & 54.9/53.6 & 25.3/23.0 & 18.5/25.4 & 17.6/11.1 \\
Qwen-14B-Chat & 64.8/67.4 & 36.9/42.6 & 33.1/51.4 & 27.6/26.8 \\
InternLM2-Chat-20B & 75.2/64.8 & 47.6/32.3 & 40.9/41.6 & 30.6/16.0 \\
Yi-34B-Chat & 62.0/67.6 & 28.6/31.6 & 26.3/35.7 & 16.5/19.1 \\
\hline
Deepseek-67B-Chat & 80.2/74.3 & 47.1/36.0 & 43.0/43.2 & 50.6/33.6 \\
Qwen-72B-Chat & 79.0/81.1 & 53.1/54.6 & 46.8/70.7 & 41.3/40.4 \\
\hline
\multicolumn{5}{c}{\textit{\greencolor{$\triangle$Mathematical Models}}} \\
MammoTH-7B & 26.8/9.4 & 8.2/1.1 & 8.5/2.5 & 6.7/0.7 \\
Metamath-Llemma-7B & 47.3/23.3 & 21.7/6.5 & 24.2/10.9 & 14.3/5.9 \\
InternLM2-Chat-Math-7B & 67.9/67.0 & 33.2/46.8 & 31.5/64.2 & 29.4/28.5 \\
Deepseek-Math-7B-Instruct & 71.5/75.8 & 33.6/39.1 & 32.8/48.7 & 27.8/32.0 \\
Deepseek-Math-7B-RL & 83.1/78.4 & 54.1/45.3 & 48.5/57.4 & 46.8/38.6 \\
MammoTH-13B & 49.6/19.9 & 17.7/3.4 & 15.1/5.0 & 15.9/5.2 \\
InternLM2-Chat-Math-20B & 69.4/69.9 & 36.4/47.2 & 33.7/68.3 & 30.8/29.1 \\
MammoTH-70B & 70.2/48.3 & 31.0/19.9 & 29.9/22.7 & 30.4/18.6 \\
\hline
\end{tabular}
\end{table*}

==> tabs/bilingual_cn.tex <==
% \begin{table*}[!thb]
% \centering
% \caption{MathBench Bilingual Score Detailed Results (Chinese)}
% \label{tab: bilingual chinese score}
% \begin{tabular}{lcccc}
% \hline
% \textbf{Models} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} \\
% \hline
% \multicolumn{5}{c}{\textit{\purplecolor{\ding{72}Closed-source Models}}} \\
% GPT-3.5 & 59.3 & 39.3 & 19.4 & 21.5 \\
% Qwen-Max & 86.2 & 75.2 & 48.4 & 45.4 \\
% GLM4 & 82.8 & 69.9 & 42.7 & 33.8 \\
% Claude-3-Opus & 86.3 & 62.5 & 37.0 & 28.2 \\
% GPT-4 & 86.6 & 72.3 & 47.2 & 54.7 \\
% \hline
% \multicolumn{5}{c}{\textit{\bluecolor{$\heartsuit$Open-source Chat Models}}} \\
% ChatGLM3-6B & 36.7 & 23.1 & 6.6 & 6.3 \\
% Yi-6B-Chat & 39.2 & 21.1 & 10.0 & 8.5 \\
% InternLM2-Chat-7B & 67.5 & 45.8 & 23.1 & 15.5 \\
% Qwen-7B-Chat & 51.4 & 40.5 & 17.6 & 15.1 \\
% Deepseek-7B-Chat & 35.2 & 14.7 & 6.2 & 8.7 \\
% \hline
% Baichuan2-13B-Chat & 53.6 & 33.7 & 14.7 & 11.1 \\
% Qwen-14B-Chat & 67.4 & 61.6 & 32.4 & 26.8 \\
% InternLM2-Chat-20B & 64.8 & 47.3 & 26.6 & 16.0 \\
% Yi-34B-Chat & 67.6 & 47.3 & 20.1 & 19.1 \\
% \hline
% Deepseek-67B-Chat & 74.3 & 49.7 & 29.5 & 33.6 \\
% Qwen-72B-Chat & 81.1 & 76.6 & 48.7 & 40.4 \\
% \hline
% \multicolumn{5}{c}{\textit{\greencolor{$\triangle$Mathematical Models}}} \\
% MammoTH-7B & 9.4 & 2.4 & 1.2 & 0.7 \\
% Metamath-Llemma-7B & 23.3 & 10.5 & 6.9 & 5.9 \\
% InternLM2-Chat-Math-7B & 67.0 & 67.5 & 43.6 & 28.5 \\
% Deepseek-Math-7B-Instruct & 75.8 & 50.8 & 37.1 & 32.0 \\
% Deepseek-Math-7B-RL & 78.4 & 60.3 & 42.4 & 38.6 \\
% MammoTH-13B & 19.9 & 3.7 & 4.6 & 5.2 \\
% InternLM2-Chat-Math-20B & 69.9 & 71.9 & 43.7 & 29.1 \\
% MammoTH-70B & 48.3 & 25.3 & 17.4 & 18.6 \\
% \hline
% \end{tabular}
% \end{table*}

\begin{table*}[!thb]
\centering
\caption{MathBench Bilingual Score Detailed Results (Chinese)}
\label{tab: bilingual english score}
\begin{tabular}{lcccc}
\hline
\textbf{Models} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} \\
\hline
\multicolumn{5}{c}{\textit{\purplecolor{\ding{72}Closed-source Models}}} \\
GPT-4o-2024-05-13 & 91.6 & 84.4 & 62.6 & 63.7 \\
GPT-3.5-turbo-0125 & 64.8 & 41.0 & 21.6 & 25.5 \\
GPT-4-0125-preview & 87.2 & 73.3 & 48.7 & 50.4 \\
Qwen-Max-0428 & 91.6 & 84.9 & 57.4 & 52.1 \\
GLM4 & 86.0 & 75.6 & 42.1 & 33.5 \\
Deepseek-v2-api & 87.6 & 75.9 & 47.9 & 44.7 \\
Claude-3-opus & 86.0 & 69.6 & 49.7 & 50.5 \\
\hline
\multicolumn{5}{c}{\textit{\bluecolor{$\heartsuit$Open-source Chat Models}}} \\
ChatGLM3-6B & 37.3 & 25.9 & 8.2 & 6.2 \\
Yi-6B-chat-lmdeploy & 39.9 & 22.8 & 9.2 & 11.9 \\
InternLM2-chat-7B & 65.1 & 51.6 & 23.4 & 19.3 \\
Qwen-7B-chat & 54.4 & 40.9 & 18.9 & 15.6 \\
Deepseek-7B-chat & 39.0 & 18.5 & 8.9 & 8.3 \\
\hline
Baichuan2-13B-chat & 54.8 & 30.2 & 21.9 & 26.9 \\
Qwen-14B-chat & 70.0 & 64.3 & 33.7 & 19.8 \\
InternLM2-chat-20B & 61.7 & 49.0 & 25.4 & 26.9 \\
Yi-34B-chat-lmdeploy & 69.4 & 48.9 & 29.7 & 35.2 \\
\hline
Deepseek-67B-chat & 73.7 & 49.3 & 36.1 & 43.1 \\
Llama-3-70B-instruct & 69.3 & 49.3 & 29.7 & 35.2 \\
Qwen-72B-chat & 82.4 & 81.0 & 50.2 & 43.8 \\
\hline
\multicolumn{5}{c}{\textit{\greencolor{$\triangle$Mathematical Models}}} \\
Mammoth-7B & 9.6 & 2.6 & 1.6 & 0.7 \\
Metamath-llemma-7B & 24.9 & 11.5 & 7.6 & 8.7 \\
InternLM2-chat-math-7B & 66.0 & 69.5 & 39.0 & 26.1 \\
Deepseek-math-7B-instruct & 75.6 & 54.3 & 40.0 & 35.5 \\
Deepseek-math-7B-rl & 80.3 & 63.2 & 43.6 & 42.6 \\
Mammoth-13B & 72.5 & 35.5 & 29.7 & 33.9 \\
InternLM2-chat-math-20B & 72.5 & 63.2 & 29.7 & 33.9 \\
Mammoth-70B & 21.3 & 4.6 & 4.6 & 5.4 \\
\hline
\end{tabular}
\end{table*}


==> tabs/bilingual_en.tex <==
\begin{table*}[!thb]
\centering
\caption{MathBench Bilingual Score Detailed Results (English)}
\label{tab: bilingual english score}
\begin{tabular}{lcccc}
\hline
\textbf{Models} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} \\
\hline
\multicolumn{5}{c}{\textit{\purplecolor{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 76.5 & 39.2 & 41.7 & 42.9 \\
Qwen-Max & 82.2 & 50.1 & 54.4 & 48.6 \\
GLM4 & 83.1 & 58.1 & 61.4 & 48.6 \\
Claude-3-Opus & 86.0 & 64.5 & 59.4 & 49.1 \\
GPT-4 & 79.1 & 67.3 & 66.1 & 63.4 \\
\hline
\multicolumn{5}{c}{\textit{\bluecolor{$\heartsuit$Open-source Chat Models}}} \\
ChatGLM3-6B & 44.4 & 19.7 & 16.4 & 6.2 \\
Yi-6B-Chat & 42.9 & 19.5 & 13.0 & 9.6 \\
InternLM2-Chat-7B & 67.4 & 36.2 & 36.2 & 29.6 \\
Qwen-7B-Chat & 48.9 & 24.8 & 22.8 & 19.5 \\
Deepseek-7B-Chat & 43.4 & 16.3 & 12.9 & 9.7 \\
\hline
Baichuan2-13B-Chat & 54.9 & 25.3 & 18.5 & 17.6 \\
Qwen-14B-Chat & 64.8 & 36.9 & 33.1 & 27.6 \\
InternLM2-Chat-20B & 75.2 & 47.6 & 40.9 & 30.6 \\
Yi-34B-Chat & 62.0 & 28.6 & 26.3 & 16.5 \\
\hline
Deepseek-67B-Chat & 80.2 & 47.1 & 43.0 & 50.6 \\
Qwen-72B-Chat & 79.0 & 53.1 & 46.8 & 41.3 \\
\hline
\multicolumn{5}{c}{\textit{\greencolor{$\triangle$Mathematical Models}}} \\
MammoTH-7B & 26.8 & 8.2 & 8.5 & 6.7 \\
Metamath-Llemma-7B & 47.3 & 21.7 & 24.2 & 14.3 \\
InternLM2-Chat-Math-7B & 67.9 & 33.2 & 31.5 & 29.4 \\
Deepseek-Math-7B-Instruct & 71.5 & 33.6 & 32.8 & 27.8 \\
Deepseek-Math-7B-RL & 83.1 & 54.1 & 48.5 & 46.8 \\
MammoTH-13B & 49.6 & 17.7 & 15.1 & 15.9 \\
InternLM2-Chat-Math-20B & 69.4 & 36.4 & 33.7 & 30.8 \\
MammoTH-70B & 70.2 & 31.0 & 29.9 & 30.4 \\
\hline
\end{tabular}
\end{table*}


==> tabs/main_results_512.tex <==
\begin{table*}[!thb]
\centering
\caption{\textbf{Overall Comparison of Chat Models on MathBench}. Models are classified into three categories according to their purpose and origin. The model name in \textbf{bold} indicates the top performer among Open-source or Closed-source models, while an \underline{underline} signifies the leading model within a similar parameter size group.}
\vspace{-2mm}
\label{tab:main_results_512}
\resizebox{\linewidth}{!}{
\tablestyle{10pt}{1.2}
\begin{tabular}{lccccc|c}
\hline
\textbf{Models} & \textbf{Arithmetic} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Average} \\
\hline
\multicolumn{7}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 70.3 & 67.9 & 39.3 & 30.6 & 32.2 & 48.1 \\
GLM4 & 61.3 & 83.0 & 64.0 & 52.1 & 41.2 & 60.3 \\
Qwen-Max & 69.3 & 84.2 & 62.7 & 51.4 & 47.0 & 62.9 \\
Claude-3-Opus & \textbf{84.7} & \textbf{86.1 }& 63.5 & 48.2 & 38.7 & 64.2 \\
GPT-4 & 76.3 & 82.9 & \textbf{69.8} & \textbf{56.6} & \textbf{59.0} & \textbf{68.9} \\
\hline
\multicolumn{7}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
Yi-6B-Chat & 35.7 & 41.1 & 20.3 & 11.5 & 9.1 & 23.5 \\
Deepseek-7B-Chat & 46.0 & 39.3 & 15.5 & 9.6 & 9.2 & 23.9 \\
ChatGLM3-6B & 41.0 & 40.5 & 21.4 & 11.5 & 6.3 & 24.1 \\
Qwen-7B-Chat & 51.3 & 50.2 & 32.6 & 20.2 & 17.3 & 34.3 \\
InternLM2-Chat-7B & \underline{53.0} & \underline{67.5} & \underline{41.0} & \underline{29.6} & \underline{22.6} & \underline{42.7} \\
\hline
Baichuan2-13B-Chat & 46.0 & 54.2 & 29.5 & 16.6 & 14.3 & 32.1 \\
Yi-34B-Chat & 51.0 & 64.8 & 38.0 & 23.2 & 17.8 & 39.0 \\
InternLM2-Chat-20B & 62.7 & \underline{70.0} & 47.4 & \underline{33.7} & 23.3 & 47.4 \\
Qwen-14B-Chat & \underline{64.7} & 66.1 & \underline{49.2} & 32.8 & \underline{27.2} & \underline{48.0} \\

\hline
Deepseek-67B-Chat & 61.3 & 77.2 & 48.4 & 36.3 & 36.8 & 52.1 \\
Qwen-72B-Chat & \textbf{72.0} & \underline{80.1} & \textbf{64.8} & \textbf{47.8} & \underline{40.8} & \textbf{61.1} \\
\hline
\multicolumn{7}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
MammoTH-7B & 26.7 & 18.1 & 5.3 & 4.8 & 3.7 & 11.7 \\
MammoTH-13B & 35.0 & 34.8 & 10.7 & 9.9 & 10.6 & 20.2 \\
Metamath-Llemma-7B & 48.7 & 35.3 & 16.1 & 15.5 & 10.1 & 25.1 \\
MammoTH-70B & 35.7 & 59.3 & 28.1 & 23.6 & 24.5 & 34.2 \\
InternLM2-Chat-Math-7B & 53.7 & 66.0 & 49.0 & 34.3 & 26.9 & 46.0 \\
Deepseek-Math-7B-Instruct & 61.0 & 73.7 & 42.2 & 34.9 & 29.9 & 48.3 \\
InternLM2-Chat-Math-20B & 58.7 & 71.1 & 55.5 & 41.8 & 31.9 & 51.8 \\
Deepseek-Math-7B-RL & \underline{67.7} & \textbf{80.8} & \underline{57.2} & \underline{45.4} & \textbf{42.7} & \underline{58.8} \\
\hline
\end{tabular}}
\end{table*}

==> tabs/theory_tab.tex <==
\begin{table*}[!htbp]
\centering
\caption{\textbf{Overall Comparison of Models on MathBench-T}. We present scores for theory questions here, the \textit{Arithmetic} and \textit{Primary} stage are combined because they share the same theory knowledge. Models are classified into three categories according to their purpose and origin. The model name in \textbf{bold} indicates the top performer among Open-source or Closed-source models, while an \underline{underline} signifies the leading model within a similar parameter size group.}
\label{tab: theory_result}
\begin{tabular}{lcccc|c}
\hline
\textbf{Models} & \textbf{Primary} & \textbf{Middle} & \textbf{High} & \textbf{College} & \textbf{Average} \\
\hline
\multicolumn{6}{c}{\purplecolor{\textit{\ding{72}Closed-source Models}}} \\
GPT-3.5 & 66.8 & 50.9 & 43.8 & 47.5 & 52.3 \\
Claude-3-Opus & 87.0 & 73.0 & 63.1 & 53.3 & 69.1 \\
GLM4 & 87.0 & 74.0 & 62.8 & 61.4 & 71.3 \\
Qwen-Max & \textbf{87.8} & 75.0 & 69.0 & 73.3 & 76.3 \\
GPT-4 & 85.4 & \textbf{78.3} & \textbf{70.9} & \textbf{79.8} & \textbf{78.6} \\
\hline
\multicolumn{6}{c}{\bluecolor{\textit{$\heartsuit$Open-source Chat Models}}} \\
Deepseek-7B-Chat & 33.0 & 26.0 & 15.4 & 16.6 & 22.8 \\
ChatGLM3-6B & 38.4 & 31.2 & 20.0 & 12.0 & 25.4 \\
Yi-6B-Chat & 46.2 & 33.3 & 19.4 & 16.8 & 28.9 \\
Qwen-7B-Chat & 51.7 & 43.3 & 30.7 & 29.1 & 38.7 \\
InternLM2-Chat-7B & \underline{67.3} & \underline{57.0} & \underline{44.9} & \underline{38.8} & \underline{52.0} \\
\hline
Baichuan2-13B-Chat & 58.1 & 44.3 & 29.9 & 25.0 & 39.3 \\
InternLM2-Chat-20B & 64.3 & 55.2 & 43.8 & 32.9 & 49.1 \\
Yi-34B-Chat & 69.3 & 52.2 & 39.0 & 32.9 & 48.4 \\
Qwen-14B-Chat & \underline{70.9} & \underline{61.8} & \underline{45.9} & \underline{46.5} & \underline{56.3} \\
\hline
Deepseek-67B-Chat & 78.1 & 63.8 & 53.5 & 60.9 & 64.1 \\
Qwen-72B-Chat & \textbf{89.4} & \textbf{76.9} & \textbf{64.9} & \underline{66.3} & \textbf{74.4} \\
\hline
\multicolumn{6}{c}{\greencolor{\textit{$\triangle$Mathematical Models}}} \\
MammoTH-7B & 11.8 & 7.6 & 8.3 & 6.3 & 8.5 \\
MammoTH-13B & 27.9 & 16.4 & 15.7 & 16.8 & 19.2 \\
Metamath-Llemma-7B & 21.2 & 23.3 & 22.0 & 16.1 & 20.7 \\
MammoTH-70B & 57.9 & 45.2 & 38.9 & 43.7 & 46.4 \\
InternLM2-Chat-Math-7B & 64.9 & 57.7 & 50.7 & 46.5 & 55.0 \\
Deepseek-Math-7B-Instruct & 73.3 & 54.7 & 48.5 & 50.2 & 56.7 \\
InternLM2-Chat-Math-20B & 72.2 & 68.0 & 59.4 & 52.5 & 63.0 \\
Deepseek-Math-7B-RL & \underline{78.9} & \underline{69.7} & \underline{59.9} & \textbf{68.0} & \underline{69.1} \\
\hline
\end{tabular}
\end{table*}






